Rapid Model Architecture Adaption for Meta-Learning

Network Architecture Search (NAS) methods have recently gathered much attention. They design networks with better performance and use a much shorter search time compared to traditional manual tuning. Despite their efficiency in model deployments, most NAS algorithms target a single task on a fixed hardware system. However, real-life few-shot learning environments often cover a great number of tasks (T ) and deployments on a wide variety of hardware platforms (H ). The combinatorial search complexity T times H creates a fundamental search efficiency challenge if one naively applies existing NAS methods to these scenarios. To overcome this issue, we show, for the first time, how to rapidly adapt model architectures to new tasks in a many-task many-hardware few-shot learning setup by integrating Model Agnostic Meta Learning (MAML) into the NAS flow. The proposed NAS method (H-Meta-NAS) is hardware-aware and performs optimisation in the MAML framework. H-Meta-NAS shows a Pareto dominance compared to a variety of NAS and manual baselines in popular few-shot learning benchmarks with various hardware platforms and constraints. In particular, on the 5-way 1-shot Mini-ImageNet classification task, the proposed method outperforms the best manual baseline by a large margin (5.21% in accuracy) using 60% less computation.

==> sections/evaluation.tex <==
\section{Evaluation}

% \begin{table*}[h!]
%   \caption{
%     Details of hardware systems experimented with \nas.}
%   \label{tab:hardware}
%   \begin{center}
%   \adjustbox{scale=0.7}{%    
%   \begin{tabular}{ccc}
%     \toprule
%     System
%     & Device 
%     & Specs 
%     \\
%     \midrule
%     Cloud
%     & Nvidia GeForce RTX 2080 Ti
%     & 4352 CUDA cores at 1635MHz
%     \\
%     Mid-end CPU 
%     & Intel CPU
%     & 2.3GHz 8-core i9 CPU (2.3GHz, 16GB RAM)
%     \\
%     Mobile CPU
%     & Raspberry Pi 4B
%     & Quad core Cortex-A72 (ARMv8) CPU (1.5GHz, 4GB RAM)
%     \\
%     IoT
%     & Raspberry Pi Zero 
%     & Single core ARM11 (ARMv6) CPU (1GHz, 512MB RAM)\\
%     ASIC
%     & Eyeriss \cite{chen2016eyeriss}
%     & 65nm with a core frequency of 250 MHz \\
%     \bottomrule
%     \end{tabular}
% }
%   \end{center}

% \end{table*}
% \begin{table}[]
%   \caption{
%     Details of hardware systems experimented with \nas.}
%   \label{tab:hardware}
%   \begin{center}
%   \adjustbox{scale=0.4}{%    
%   \begin{tabular}{c|ccccc}
%     \toprule
%     System
%     & Cloud
%     & Mid-end CPU
%     & Mobile CPU
%     & IoT
%     & ASIC
%     \\
%     Device 
%     & Nvidia GeForce RTX 2080 Ti
%     & Intel CPU
%     & Raspberry Pi 4B
%     & Raspberry Pi Zero 
%     & Eyeriss \cite{chen2016eyeriss}
%     \\
%     \bottomrule
%     \end{tabular}
% }
%   \end{center}
% \end{table}

\begin{table}[]
  \caption{
    Details of hardware systems experimented with \nas.}
  \label{tab:hardware}
  \begin{center}
  \adjustbox{scale=0.7}{%    
  \begin{tabular}{cc}
    \toprule
    System
    & Device 
    \\
    \midrule
    Cloud
    & Nvidia GeForce RTX 2080 Ti
    \\
    Mid-end CPU 
    & Intel CPU
    \\
    Mobile CPU
    & Raspberry Pi 4B
    \\
    IoT
    & Raspberry Pi Zero 
    \\
    ASIC
    & Eyeriss \cite{chen2016eyeriss}
    \\
    \bottomrule
    \end{tabular}
}
  \end{center}
\vspace{-15pt}
\end{table}

We evaluate \nas~in a few-shot learning setup.
For each dataset, we search for the meta-architecture and meta-parameters.
We then adapt the meta-architecture with respect to a target hardware-constraint pair.
In the evaluation stage, we then re-train the obtained hardware-aware task-specific architecture to convergence and report the final accuracy.
We consider three popular datasets in the few-shot learning community: Omniglot, Mini-ImageNet and Few-shot CIFAR100. We use the PytorchMeta framework to handle the datasets \citep{deleu2019torchmeta}.

\textbf{Omniglot} is a handwritten digits recognition task, containing 1623 samples \citep{lake2015human}. 
We use the meta train/validation/test splits used Vinyals \etal~\cite{vinyals2016matching}. These splits are over 1028/172/423 classes (characters).

\textbf{Mini-ImageNet} is first introduced by Vinyals \etal. 
This dataset contains images of 100 different classes from the ILSVRC-12 dataset \citep{deng2009imagenet}, the splits are taken from Ravi \etal \citep{ravi2016optimization}.

\textbf{FC100} is introduced by \citeauthor{oreshkin2018tadam}, the datasets has 100 different classes from the CIFAR100 dataset \cite{krizhevsky09learningmultiple}.

\Cref{tab:hardware} details the systems and representative devices considered. Our Appendix contains a more detailed explanation of the specs of each hardware device. We use the ScaleSIM cycle-accurate simulator \cite{samajdar2018scale} for the Eyeriss \cite{chen2016eyeriss} accelerator. Details about this simulation and more information with respect to the datasets and search configurations are in our Appendix. 

% \begin{figure}[!h]
% 	\begin{center}
%         \includegraphics[width=\linewidth]{scripts/frontier_size.pdf}
% 	\end{center}
% 	\caption{
%         Deploying networks to different tasks with various constraint-hardware paris. This implies a huge search space $N \times M \times K$, and requires a huge amount of manual architectural engineering time.
% 		}
% 	\label{fig:cora}
% \end{figure}
% \vspace{-20pt}
\paragraph{The effect of pool sizes}
\begin{figure}[]
	\centering
	\includegraphics[width=.9\linewidth]{scripts/pool_size_ablation.pdf}
	\caption{The effect of different pool size (P) and different number of iterations (M).}
	\label{fig:pool}
  \vspace{-15pt}
\end{figure}
We identify the following two hyper-parameters that can potentially affect the performance in the adaption stage, namely the number of iterations $M$ and the pool size $P$, and then run an hyper-parameter analysis in \Cref{fig:pool}. The full adaption algorithm making use of these hyper-parameters is in our Appendix. The horizontal axis shows the number of iterations and the vertical axis shows the averaged accuracy on the sampled tasks for all architectures in the pool.
\Cref{fig:pool} shows that the accuracy convergence is reached after around $150$ iterations, and running for additional iterations only provides marginal accuracy gains.
For this reason, we picked the number of iterations to be $200$ for a balance between accuracy and run-time.
In the meantime, we notice in general a higher pool size will give better adapted accuracy. However, 
this does not mean the final searched accuracy is affected to the same degree.
The final re-trained accuracies of searched architectures show an accuracy gap of $0.21\%$ between $P=100$ and $P=200$ and $0.32\%$ between $P=100$ and $P=500$.
An increase in pool size can prolong the run-time significantly, we thus picked a pool size of $100$ since it offers the best balance between accuracy and run-time.

\input{tables/vgg_case_study.tex}
% \vspace{-10pt}
\paragraph{Evaluating pooling, GE and ANL}
Our results in \Cref{tab:case_study} suggest that a correct pooling strategy, GE and ANL can change the NAS backbone to allow the search space to reach much smaller models and thus provide a better accuracy.
In addition, \Cref{tab:case_study} also illustrates that $5 \times 5$ pooling is necessary for a higher accuracy.
We hypothesize this is because a relatively large fully-connected layer after the pooling is required for the network to achieve a good accuracy in this few-learning setup. 


\paragraph{Latency predictor \vs~layer-wise latency profiling}
\input{tables/latency_predictor.tex}
We re-implemented the latency predictor in OFA \cite{cai2019once} to illustrate how a layer-wise profiling and look-up method is a perfect match in our learning scenario. We pick 16K training samples and 10K validation samples to train and test the latency predictor, which is the same as setup used in OFA. We use another 10K testing samples to evaluate the performance of OFA-based latency predictor against our layer-wise profiling on different hardware systems in terms of MSE (measuring the latency estimation quality) and Time (measuring the efficiency).

As illustrated in \Cref{tab:latency}, layer-wise profiling saves not only time but also has a smaller MSE error compared to a predictor-based strategy that is very popular in today's evolutionary-based NAS frameworks \citep{cai2019once, cai2018proxylessnas}. In addition, layer-wise profiling shows orders of magnitude better run-time when targeting hardware devices with scarce computational resources. If we consider an IoT class device as a target (i.e the Raspberry Pi Zero), it requires an unreasonably large amount of time to generate training samples for latency predictors, making them an infeasible approach in real life. For instance, the total time consumed by latency predictor is infeasible to execute on Pi Zero (last row in \Cref{tab:latency}). Of course, in reality, there is also a great number of IoT devices using more low-end CPUs compared to Pi Zero (ARMV5 or ARMV4), making the latency predictor even harder to be deployed on these devices. Also in a many-hardware setup considered in this paper, this profiling is executed O(H) times.

Most existing layer-wise look-up approaches consider at most mobile systems as targeting platforms \citep{xu2020latency,yang2018netadapt}. These systems are in general more capable than a great range of IoT devices. In this paper, we demonstrate the effectiveness of this approach on more low-end systems (Raspberry Pi and Pi Zeros), illustrating this is the more scalable approach for hardware-aware NAS for constrained hardware systems.


\paragraph{Evaluating \nas~searched architectures}
\label{sec:eval:nas}
\input{tables/omniglot.tex}
\input{tables/miniimagenet.tex}

\Cref{tab:omniglot} displays the results of \nas~on the Omniglot 20-way 1-shot and 5-shot classification tasks. 
We match the size of \nas~to MAML and MAML++ for a fair comparison.
\nas~outperforms all competing methods apart from the original MAML++.
MAML++ uses a special evaluation strategy, it creates an ensemble of models with best validation-set performance. 
MAML++ then picks the best model from the ensemble based on support set loss and report accuracy on the query set.
We then locally replicated MAML++ without this trick, and show that \nas~outperforms it by a significant margin ($+1.01\%$ on 1-shot and $+0.11\%$ on 5-shot) with around half of the MACs ($4.95G$ compared to $10.07G$).

\Cref{tab:miniimagenet} shows the results of running the 5-way 1-shot and 5-shot Mini-ImageNet tasks, similar to the previous results, we match the size of searched networks to MAML, MAML++ and ALFA+MAML+L2F.
\Cref{tab:miniimagenet} not only displays results on MAML methods with fixed-architectures, it also shows the performance of searched networks including Auto-Meta \cite{kim2018auto}, BASE \cite{shaw2018meta} and T-NAS \cite{lian2019towards}.
\nas~shows interesting results when compared to T-NAS and T-NAS++. 
\nas~has a much higher accuracy ($+3.26\%$ in 1-shot and $7.94\%$ in 5-shot) and a smaller MAC count, but uses a greater amount of parameters.
T-NAS and T-NAS++ use DARTS cells \cite{liu2018darts}.
This NAS cell contains a complex routing of computational blocks, making it not suitable for latency critical applications.
We will demonstrate later how this design choice gives 
a worse on-device latency performance.
We also show how \nas~work with FC100 in Appendix.

\paragraph{\nas~for diverse hardware platforms and constraints}
\label{sec:eval:latency}
\begin{figure}[]
  \centering
    \centering
    \includegraphics[width=.9\linewidth]{scripts/frontier_gpu_lat.pdf}
    \caption{Targeting a GPU}
    \label{fig:gpu}
  \caption{Applying \nas~with GPU latency as optimisation targets.}
  \label{fig:sizes:gpus}
  \vspace{-15pt}
\end{figure}

In addition to using the model sizes as a constraint for \nas, we use various latency targets on various hardware platforms as the optimisation target.
\Cref{fig:sizes:gpus} shows how GPU latencies can be used as constraints.
% T-NAS and T-NAS++ show a better performance on the size-accuracy plot in \Cref{fig:sizes}.
The smaller model sizes of T-NAS do not provide a better run-time on GPU devices (\Cref{fig:gpu}), in fact, T-NAS based models have the worst run-time on GPU devices due to the complicated dependency of DARTS cells. 
% \Cref{fig:cpu:asic:iot} illustrates the performance of \nas~on different CPU devices and an ASIC hardware. The details of these hardware are described in \Cref{tab:hardware}.
% In \Cref{fig:cpu:asic:iot}, \nas~shows a better Pareto-frontier performance compared to a range of baselines and searched models.
We only compare to MAML and MAML++ when running on Eyeriss due to the limitations of the ScaleSIM simulator \cite{samajdar2018scale}.
In our Appendix, we provide more latency \vs~accuracy plots using various hardware platforms' latency as constraints and observe the same pareto dominance shown in \Cref{fig:sizes:gpus}.
% Our results in both \Cref{fig:sizes:gpus} and \Cref{fig:cpu:asic:iot} demonstrate that \nas~consistently generates more efficient models compared to various MAML-based methods.


% \begin{figure}
%     \centering
%     \begin{subfigure}{.5\textwidth}
%       \centering
%       \includegraphics[width=.95\linewidth]{scripts/frontier_asic_lat.pdf}
%       \caption{Targeting an ASIC accelerator}
%       \label{fig:asic}
%     \end{subfigure}%
%     \begin{subfigure}{.5\textwidth}
%       \centering
%       \includegraphics[width=.95\linewidth]{scripts/frontier_cpu_lat.pdf}
%       \caption{Targeting a mid-end CPU}
%       \label{fig:midcpu}
%     \end{subfigure}

%     \vskip\baselineskip
%     \begin{subfigure}{.5\textwidth}
%       \centering
%       \includegraphics[width=.95\linewidth]{scripts/frontier_pi4b_lat.pdf}
%       \caption{Targeting a low-end CPU} 
%       \label{fig:lowcpu}
%     \end{subfigure}%
%     \begin{subfigure}{.5\textwidth}
%       \centering
%       \includegraphics[width=.95\linewidth]{scripts/frontier_pizero_lat.pdf}
%       \caption{Targeting an IoT device}
%       \label{fig:iot}
%     \end{subfigure}
%     \caption{Applying \nas~with ASIC and CPUs as targets.}
%     \label{fig:cpu:asic:iot}
% \end{figure}


\input{tables/backbone_algorithm.tex}  
\input{tables/search_time.tex}

\paragraph{A more complex NAS backbone}
\Cref{tab:complicate} shows how \nas~performs with a more complicated NAS backbone.
In previous experiments, we build the NAS on top of a VGG9 backbone since it is the architecture utilised in the MAML++ algorithm.
For the purpose of having a fair comparison, we did not manually pick a complex NAS backbone.
However, we demonstrate, in this section, that \nas~can be applied with a more complicated backbone and it shows better final accuracy as expected.
The trained accuracy of searched networks using ResNet12 reaches a $7.31\%$ higher accuracy compared the original VGG9 backbone.
In addition, we compare the proposed approach with state-of-the-art Metric-based meta-learning methods \cite{zhang2020deepemd,chen2020new}.
Although using only a single inference pass (our method does not conduct inference runs on the support set when deployed), \nas~shows competitive results with SOTA Metric-based methods while having a much smaller MACs usage (around $20 \times$).
\paragraph{Search complexity and search time}
In \Cref{tab:searchtime}, we show a comparison between \nas~and various NAS schemes in the many-task many-device setup. Specifically, we consider a scenario with $500$ tasks and 10 different hardware-constraint paris.
Our results in \Cref{tab:searchtime} suggest that \nas~is the most efficient search method because of its low search complexity.

% In \Cref{tab:searchtime}, we show how \nas~compares to various NAS schemes in the many-task many-device setup. Specifically, we consider a scenario with $500$ tasks and 10 different hardware-constraint paris.
% Our results in \Cref{tab:searchtime} suggest that \nas~is the most efficient search method because of its low search complexity.

